VesNet: Neural network accelerated solver for simulating Stokesian vesicle suspensions

Numerical simulation of deformable particle suspensions in Stokes flow is computationally expensive due to nonlinear fluid-structure interactions, evolving interfaces, and multiscale hydrodynamics. We present VesNet, a hybrid framework that accelerates two-dimensional vesicle suspension simulations by approximating vesicle self interactions, including background flow coupling and short-range lubrication forces, while retaining conventional modules for boundary reparameterization and far-field hydrodynamics. A GPU-accelerated implementation achieves over 100x speedup compared to a multithreaded MATLAB CPU boundary integral solver and about 5x relative to its GPU counterpart. VesNet accurately captures key dynamics, including single-vesicle phase behavior, pair interactions, and large-scale suspensions in Taylor-Green and Poiseuille flows, enabling efficient simulations of thousands of vesicles on modest computational resources.

==> Makefile <==
main=main_vesnet
summaryf=summary
compile=pdflatex

all:
	${compile} ${main}
	${compile} ${main}
	bibtex ${main}
	${compile} ${main}
	${compile} ${main}
	@echo Done ....!

pdf:
	${compile} ${main}

bib:
	${compile} ${main}
	bibtex ${main}

clean:
	rm -f *.aux *.log *.dvi *.blg *.bbl \
          *.fls *.fdb_latexmk *.out     \
          *.brf *.snm *.toc *.nav       \
		  *.pdfsync *synctex.gz 
	@echo Cleaned ....! 

cleanpdf:
	mv *.pdf /tmp 
	@echo Cleaned pdfs!

